Deep Policy Iteration with Integer Programming for Inventory Management

We present a Reinforcement Learning (RL) based framework for optimizing long-term discounted reward problems with large combinatorial action space and state dependent constraints. These characteristics are common to many operations management problems, e.g., network inventory replenishment, where managers have to deal with uncertain demand, lost sales, and capacity constraints that results in more complex feasible action spaces. Our proposed Programmable Actor Reinforcement Learning (PARL) uses a deep-policy iteration method that leverages neural networks (NNs) to approximate the value function and combines it with mathematical programming (MP) and sample average approximation (SAA) to solve the per-step-action optimally while accounting for combinatorial action spaces and state-dependent constraint sets. We show how the proposed methodology can be applied to complex inventory replenishment problems where analytical solutions are intractable. We also benchmark the proposed algorithm against state-of-the-art RL algorithms and commonly used replenishment heuristics and find it considerably outperforms existing methods by as much as 14.7% on average in various complex supply chain settings. We find that this improvement of PARL over benchmark algorithms can be directly attributed to better inventory cost management, especially in inventory constrained settings. Furthermore, in the simpler setting where optimal replenishment policy is tractable or known near optimal heuristics exist, we find that the RL approaches can learn near optimal policies. Finally, to make RL algorithms more accessible for inventory management researchers, we also discuss the development of a modular Python library that can be used to test the performance of RL algorithms with various supply chain structures and spur future research in developing practical and near-optimal algorithms for inventory management problems.

==> code/env1s3r_cfg.tex <==
[conf_type]
conf_type = list # list for 1sMr, graph works for both pdr and 1sMr

[env_params]
env_type = 1sMr # 1sMr or pdr
state_rep = N
action_rep = MD
quant = 1
reset_max_entity_inv = 4
reset_max_connection_inv = 4
start_inventory = random # random or zero
prod_start_inventory = -1 # if below 0, set equal to prod_holding_cap

[supply_chain_params]
max_order_action = 50
prod_daily_prod_avg = 10
prod_daily_prod_std = 0
demand_avg_list = 2, 2, 2
demand_std_list = 10, 10, 10
L_list = 1, 2, 3
revenue_list = 50, 50, 50
holding_cost_list = 1, 2, 4
order_cost_per_item_list = 0, 0, 0
order_cost_fixed_list = 50, 50, 50
retailer_overorder_penalty_list = 10, 10, 10
prod_holding_capacity = 100

==> code/env_pdr_1s2w3r_cfg.tex <==
[conf_type]
conf_type = graph # specify network via graph or list

[env_params]
env_type = pdr # pdr (define producers, distributors, and retailers)
state_rep = N
action_rep = MD
quant = 1
reset_max_entity_inv = 4
reset_max_connection_inv = 4
back_order = False #Set to True for back order setting instead of lost sales


[supply_chain_general_params]
max_order_action = 50

[supply_chain_producer_params]
id_list = P1
prod_daily_prod_avg_list = 10
prod_daily_prod_std_list = 0
holding_cost_list = 0
holding_capacity_list = 100
overorder_penalty_list = 0
max_start_inv = -1 # if below 0, set equal to prod_holding_cap

[supply_chain_distributor_params]
id_list = D1, D2
holding_cost_list = 0.5, 0.5
holding_capacity_list = 150, 150
overorder_penalty_list = 10, 10
max_start_inv = 60, 60

[supply_chain_retailer_params]
id_list = R1, R2, R3
demand_avg_list = 2, 2, 2
demand_std_list = 10, 10, 10
revenue_list = 50, 50, 50
holding_cost_list = 1, 2, 4
overorder_penalty_list = 10, 10, 10
holding_capacity_list = 50, 50, 50
max_start_inv = 12, 12, 12
backorder_penalty_list = 0, 0, 0

[supply_chain_connection_params]
upstream_id_list = P1, P1, D1, D1, D2
downstream_id_list = D1, D2, R1, R2, R3
L_list = 2, 2, 1, 2, 3
order_cost_per_item_list = 0, 0, 0, 0, 0
order_cost_fixed_list = 0, 0, 50, 50, 50
max_start_inv = 6, 6, 6, 6, 6
